Bayesian Games with Intentions

We show that standard Bayesian games cannot represent the full spectrum of belief-dependent preferences. However, by introducing a fundamental distinction between intended and actual strategies, we remove this limitation. We define Bayesian games with intentions, generalizing both Bayesian games and psychological games, and prove that Nash equilibria in psychological games correspond to a special class of equilibria as defined in our setting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{99}
\providecommand{\publicationstatus}{R. Ramanujam (Ed.): TARK 2015\\
EPTCS 215, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.215.8}{10.4204/EPTCS.215.8}}

